Robust Multivariate Time-Series Forecasting: Adversarial Attacks and Defense Mechanisms

This work studies the threats of adversarial attack on multivariate probabilistic forecasting models and viable defense mechanisms. Our studies discover a new attack pattern that negatively impact the forecasting of a target time series via making strategic, sparse (imperceptible) modifications to the past observations of a small number of other time series. To mitigate the impact of such attack, we have developed two defense strategies. First, we extend a previously developed randomized smoothing technique in classification to multivariate forecasting scenarios. Second, we develop an adversarial training algorithm that learns to create adversarial examples and at the same time optimizes the forecasting model to improve its robustness against such adversarial simulation. Extensive experiments on real-world datasets confirm that our attack schemes are powerful and our defense algorithms are more effective compared with baseline defense mechanisms.

==> algorithms/alg_minimax.tex <==
\begin{algorithm}
\caption{Minimax Defense
% \youngsuk{maybe we don't need this algorithmic form as we are just solving Eq (4.3.) if out of page limit. And there are even various ways to solve it.}
}\label{alg:defense}
\begin{algorithmic}
\State \textbf{input: } dataset $\mathcal{D}$ of $(\mf{x,z})$ pairs and other parameters: 
% \youngsuk{@linbo, other para., e.g. $\mathcal{I}$?}
\begin{itemize}[leftmargin=*]
\item sparse constraint $\kappa$ for $q$ in Eq.~\eqref{eq:minimax2}
\item number of optimization iterations $n$ 
\end{itemize}
\State \textbf{output: } robust forecasting model $p_\theta(\mf{z}\mid \mf{x})$.
\For{$1,2,\ldots,n$}
\State 3. Fix $\theta$, minimize $-\sum_{(\mf{x,z})\sim\mathcal{D}}\ell_g(\phi; \mf{x, z}, \theta)$ with respect to $\phi$ -- see Eq.~\eqref{eq:minimax1}
\State 4. Fix $\phi$, maximize $\sum_{(\mf{x,z})\sim\mathcal{D}}\ell_p(\theta; \mf{x, z}, \phi)$ with respect to $\theta$ -- see Eq.~\eqref{eq:minimax2}
\EndFor
\end{algorithmic}
\end{algorithm}


==> algorithms/alg_rs.tex <==
\begin{algorithm}
% \centering
\caption{Randomized Smoothing}
\label{alg:rs}
\begin{algorithmic}
\State \textbf{input: } pre-trained $\tau$-step forecasting model $p_\theta(\mf{z}\mid \mf{x})$, observation $\mf{x}$ and other parameters  
\begin{itemize}[leftmargin=*]
\item number of samples $n$
\item noise level $\sigma$
\end{itemize}
\State \textbf{output: } $n$ sample paths $[\mf{\hat x}_{T+1:T+\tau}]_i^{(j)}$ for $i=1,\dots,d$ and $j=1,\dots,n$
\For{$j=1,2,\ldots,n$}
\State 1. Sample $\xi_{i,t}\sim\mb{N}(0,\sigma^2)$ i.i.d. and compute $\tilde x_{i,t}\gets x_{i,t}+\xi_{i,t}$
\State 2. Sample $[\mf{\hat x}_{T+1:T+\tau}]_i^{(j)}\sim p_\theta(\mf{z}\mid \mf{\tilde x})$
\EndFor
\end{algorithmic}
\end{algorithm}


==> tables/table_electricity_comp.tex <==


\begin{table*}[h]
\caption{Metrics on electricity dataset under \textbf{deterministic} attack. Target time series $I=\{1, 5\}$ and attacked time stamp $H=\{\tau-1, \tau\}$. Smaller is better.}
\label{table:electricity_i5}
\begin{center}
\begin{small}
\scalebox{0.5}{
\begin{tabular}{ccccccccccccc}
\hline
 & \multicolumn{3}{c}{no defense} & \multicolumn{3}{c}{data augmentation} & \multicolumn{3}{c}{randomized smoothing} &\multicolumn{3}{c}{mini-max defense}\\
\hline
Sparsity & WAPE & WSE & wQL & WAPE & WSE & wQL & WAPE & WSE & wQL & WAPE & WSE & wQL\\
\hline
no attack & 0.1616$\pm$0.1553 & 0.0701$\pm$0.1488 & 0.0722$\pm$0.0161& 0.1309$\pm$0.0912 & 0.0323$\pm$0.0366 & 0.0652$\pm$0.0118& 0.1395$\pm$0.0962 & 0.0363$\pm$0.0438 & 0.0676$\pm$0.0124& 0.1405$\pm$0.0884 & 0.0340$\pm$0.0381 & 0.0674$\pm$0.0229\\
1 & 0.2062$\pm$0.1542 & 0.0858$\pm$0.1531 & 0.1061$\pm$0.0450& 0.1527$\pm$0.1168 & 0.0482$\pm$0.0688 & 0.0668$\pm$0.0116& 0.1615$\pm$0.1246 & 0.0544$\pm$0.0748 & 0.0708$\pm$0.0115& 0.2025$\pm$0.1093 & 0.0628$\pm$0.0672 & 0.1116$\pm$0.0242\\
3 & 0.3467$\pm$0.1849 & 0.1825$\pm$0.2352 & 0.2238$\pm$0.0641& 0.2815$\pm$0.1484 & 0.1194$\pm$0.1317 & 0.1621$\pm$0.0800& 0.2805$\pm$0.1527 & 0.1212$\pm$0.1380 & 0.1638$\pm$0.0829& 0.3482$\pm$0.1508 & 0.1627$\pm$0.1461 & 0.2661$\pm$0.0318\\
5 & 0.5088$\pm$0.2429 & 0.3663$\pm$0.3993 & 0.3560$\pm$0.0914& 0.5386$\pm$0.2253 & 0.3826$\pm$0.3279 & 0.3968$\pm$0.0772& 0.5439$\pm$0.2289 & 0.3914$\pm$0.3430 & 0.3953$\pm$0.0802& 0.4798$\pm$0.1828 & 0.2911$\pm$0.2239 & 0.3888$\pm$0.0326\\
7 & 0.6725$\pm$0.2643 & 0.5795$\pm$0.5012 & 0.5091$\pm$0.0898& 0.7458$\pm$0.3227 & 0.7460$\pm$0.6789 & 0.5827$\pm$0.0791& 0.7452$\pm$0.3234 & 0.7459$\pm$0.6661 & 0.5841$\pm$0.0818& 0.6045$\pm$0.2082 & 0.4445$\pm$0.2963 & 0.5217$\pm$0.0754\\
9 & 0.8496$\pm$0.3179 & 0.9060$\pm$0.7161 & 0.6643$\pm$0.1018& 0.8834$\pm$0.3756 & 1.0374$\pm$0.9157 & 0.6977$\pm$0.0822& 0.8674$\pm$0.3644 & 0.9942$\pm$0.8474 & 0.6836$\pm$0.0810& 0.6977$\pm$0.2350 & 0.5874$\pm$0.3608 & 0.6570$\pm$0.0845\\
full attack & 1.0318$\pm$0.3917 & 1.3441$\pm$1.1498 & 0.7534$\pm$0.1085& 0.9354$\pm$0.3970 & 1.1623$\pm$1.0327 & 0.7644$\pm$0.0808& 0.9353$\pm$0.3945 & 1.1585$\pm$1.0326 & 0.7630$\pm$0.0823& 1.0132$\pm$0.3224 & 1.2160$\pm$0.7722 & 0.8042$\pm$0.0925\\
\hline
\end{tabular}
}
\end{small}
\end{center}
\end{table*}


==> tables/table_electricity_i5.tex <==

\begin{table*}[h]
\caption{Metrics on electricity dataset under \textbf{deterministic} attack. Target time series $I=\{5\}$ and attacked time stamp $H=\{\tau\}$. Smaller is better.}
\label{table:electricity_i5}
\begin{center}
\begin{small}
\scalebox{0.5}{
\begin{tabular}{ccccccccccccc}
\hline
 & \multicolumn{3}{c}{no defense} & \multicolumn{3}{c}{data augmentation} & \multicolumn{3}{c}{randomized smoothing} &\multicolumn{3}{c}{mini-max defense}\\
\hline
Sparsity & WAPE & WSE & wQL & WAPE & WSE & wQL & WAPE & WSE & wQL & WAPE & WSE & wQL\\
\hline
no attack & 0.0716$\pm$0.0486 & 0.0094$\pm$0.0092 & 0.0629$\pm$0.0255& 0.0633$\pm$0.0413 & 0.0071$\pm$0.0078 & 0.0564$\pm$0.0219& 0.0768$\pm$0.0429 & 0.0093$\pm$0.0102 & 0.0611$\pm$0.0251& 0.0752$\pm$0.0481 & 0.0099$\pm$0.0113 & 0.0554$\pm$0.0346\\
1 & 0.1315$\pm$0.0580 & 0.0234$\pm$0.0170 & 0.0960$\pm$0.0359& 0.1012$\pm$0.0500 & 0.0148$\pm$0.0132 & 0.0771$\pm$0.0323& 0.0961$\pm$0.0439 & 0.0127$\pm$0.0101 & 0.0714$\pm$0.0249& 0.1214$\pm$0.0942 & 0.0309$\pm$0.0335 & 0.1009$\pm$0.0792\\
3 & 0.2999$\pm$0.0717 & 0.0993$\pm$0.0444 & 0.2273$\pm$0.0638& 0.2191$\pm$0.1006 & 0.0665$\pm$0.0498 & 0.1701$\pm$0.0836& 0.2255$\pm$0.0990 & 0.0687$\pm$0.0468 & 0.1749$\pm$0.0806& 0.3285$\pm$0.1200 & 0.1341$\pm$0.0885 & 0.2774$\pm$0.1190\\
5 & 0.5498$\pm$0.1006 & 0.3208$\pm$0.1036 & 0.4656$\pm$0.0964& 0.5082$\pm$0.1297 & 0.2889$\pm$0.1300 & 0.4376$\pm$0.1218& 0.4949$\pm$0.1317 & 0.2766$\pm$0.1296 & 0.4192$\pm$0.1268& 0.6328$\pm$0.1271 & 0.4299$\pm$0.1609 & 0.5833$\pm$0.1295\\
7 & 0.7341$\pm$0.1704 & 0.5918$\pm$0.2759 & 0.6539$\pm$0.1620& 0.7204$\pm$0.1773 & 0.5763$\pm$0.2770 & 0.6407$\pm$0.1714& 0.7131$\pm$0.1766 & 0.5653$\pm$0.2693 & 0.6321$\pm$0.1683& 0.8675$\pm$0.1421 & 0.7894$\pm$0.2693 & 0.8174$\pm$0.1412\\
9 & 0.9969$\pm$0.1412 & 1.0301$\pm$0.2880 & 0.9093$\pm$0.1370& 0.9008$\pm$0.1615 & 0.8589$\pm$0.2758 & 0.8131$\pm$0.1528& 0.9083$\pm$0.1609 & 0.8721$\pm$0.2807 & 0.8225$\pm$0.1569& 1.0287$\pm$0.1307 & 1.0893$\pm$0.2830 & 0.9770$\pm$0.1275\\
full attack & 1.0541$\pm$0.1466 & 1.1502$\pm$0.3117 & 0.9655$\pm$0.1416& 0.9907$\pm$0.1743 & 1.0369$\pm$0.3063 & 0.9024$\pm$0.1656& 0.9834$\pm$0.1737 & 1.0221$\pm$0.3109 & 0.8941$\pm$0.1648& 1.1181$\pm$0.1361 & 1.2838$\pm$0.3247 & 1.0619$\pm$0.1284\\
\hline
\end{tabular}
}
\end{small}
\end{center}
\end{table*}


==> tables/table_electricity_i5_sparse.tex <==
\begin{table*}[h]
\caption{Metrics on electricity dataset under \textbf{probabilistic} attack using sparse layer.  Target time series $I=\{5\}$ and attacked time stamp $H=\{\tau\}$. Smaller is better.}
\label{table:electricity_i5_sparse}
\begin{center}
\begin{small}
\scalebox{0.5}{
\begin{tabular}{ccccccccccccc}
\hline
& \multicolumn{3}{c}{No defense} & \multicolumn{3}{c}{data augmentation} & \multicolumn{3}{c}{randomized smoothing} & \multicolumn{3}{c}{mini-max defense}\\
\hline
Sparsity & WAPE & WSE & wQL & WAPE & WSE & wQL & WAPE & WSE & wQL & WAPE & WSE & wQL\\
\hline
no attack & 0.0787$\pm$0.0513 & 0.0110$\pm$0.0115 & 0.0657$\pm$0.0383& 0.0799$\pm$0.0408 & 0.0094$\pm$0.0084 & 0.0646$\pm$0.0348& 0.0722$\pm$0.0381 & 0.0079$\pm$0.0079 & 0.0578$\pm$0.0314& 0.0731$\pm$0.0564 & 0.0112$\pm$0.0141 & 0.0563$\pm$0.0446\\
1 & 0.1590$\pm$0.0593 & 0.0317$\pm$0.0207 & 0.1117$\pm$0.0592& 0.1563$\pm$0.0821 & 0.0367$\pm$0.0322 & 0.1201$\pm$0.0729& 0.1526$\pm$0.0827 & 0.0357$\pm$0.0326 & 0.1150$\pm$0.0745& 0.1791$\pm$0.0867 & 0.0458$\pm$0.0376 & 0.1426$\pm$0.0867\\
3 & 0.3186$\pm$0.1809 & 0.1611$\pm$0.1297 & 0.2721$\pm$0.1855& 0.2893$\pm$0.1327 & 0.1158$\pm$0.0851 & 0.2258$\pm$0.1369& 0.2936$\pm$0.1250 & 0.1147$\pm$0.0817 & 0.2314$\pm$0.1351& 0.3235$\pm$0.1559 & 0.1489$\pm$0.1297 & 0.2759$\pm$0.1884\\
5 & 0.5829$\pm$0.1250 & 0.3682$\pm$0.1447 & 0.4997$\pm$0.1755& 0.4595$\pm$0.1499 & 0.2521$\pm$0.1613 & 0.3854$\pm$0.1797& 0.4577$\pm$0.1513 & 0.2512$\pm$0.1579 & 0.3840$\pm$0.1761& 0.5900$\pm$0.1516 & 0.3900$\pm$0.1985 & 0.5388$\pm$0.2334\\
7 & 0.6993$\pm$0.0772 & 0.4999$\pm$0.1039 & 0.6193$\pm$0.1830& 0.6527$\pm$0.1286 & 0.4562$\pm$0.2014 & 0.5769$\pm$0.2058& 0.6436$\pm$0.1164 & 0.4389$\pm$0.1753 & 0.5629$\pm$0.1891& 0.7185$\pm$0.1043 & 0.5361$\pm$0.1414 & 0.6758$\pm$0.2469\\
9 & 0.8304$\pm$0.1177 & 0.7147$\pm$0.2039 & 0.7482$\pm$0.2446& 0.7408$\pm$0.1250 & 0.5772$\pm$0.1909 & 0.6609$\pm$0.2203& 0.7312$\pm$0.1346 & 0.5677$\pm$0.2068 & 0.6500$\pm$0.2235& 0.9728$\pm$0.1013 & 0.9651$\pm$0.2096 & 0.9321$\pm$0.3350\\
\hline
\end{tabular}
}
\end{small}
\end{center}
\end{table*}


==> tables/table_electricity_short.tex <==
\begin{table*}[h]
\caption{Average wQL on electricity dataset under \textbf{deterministic} attack. Target time series $I=\{1\}$ and attacked time stamp $H=\{\tau\}$. Smaller is better.}
\label{table:electricity}
\begin{center}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{ccccccccccccc}
\hline
\multicolumn{5}{c}{deterministic attack}\\
\hline
Sparsity & no defense & data augmentation & randomized smoothing & mini-max defense\\
\hline
no attack & 0.2853$\pm$0.0825& 0.2288$\pm$0.0792& 0.2176$\pm$0.0700& \textbf{0.2154}$\pm$0.0705\\
1 & 0.3410$\pm$0.0946& 0.2949$\pm$0.0716& \textbf{0.2826}$\pm$0.0718& 0.2990$\pm$0.0772\\
3 & 0.4559$\pm$0.1344& \textbf{0.3655}$\pm$0.1097& 0.3757$\pm$0.1012& 0.3775$\pm$0.0923\\
5 & 0.5770$\pm$0.1772& 0.5554$\pm$0.1636& 0.5560$\pm$0.1751& \textbf{0.5273}$\pm$0.1558\\
7 & 0.6687$\pm$0.2131& 0.7076$\pm$0.2321& 0.7072$\pm$0.2308& \textbf{0.6506}$\pm$0.2111\\
9 & 0.8282$\pm$0.2847& 0.8412$\pm$0.2896& 0.8327$\pm$0.2786& \textbf{0.7503}$\pm$0.2588\\
% full attack & 1.0159$\pm$0.3542& \textbf{0.8023}$\pm$0.2664& 0.8133$\pm$0.2659& 0.9415$\pm$0.3424\\
\hline
\end{tabular}
}
\end{small}
\end{center}
\end{table*}


==> tables/table_electricity_sparse_short.tex <==
\begin{table*}[h!]
\caption{Metrics on electricity dataset under \textbf{probabilistic} attack using sparse layer.  Target time series $I=\{1\}$ and attacked time stamp $H=\{\tau\}$. Smaller is better.}
\label{table:electricity_sparse}
\begin{center}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{ccccccccccccc}
\hline
Sparsity & no defense & data augmentation & randomized smoothing & mini-max defense\\
\hline
no attack & 0.2909$\pm$0.0748& 0.2374$\pm$0.0764& \textbf{0.2237}$\pm$0.0750& 0.2342$\pm$0.0710\\
1 & \textbf{0.4364}$\pm$0.1296& 0.5923$\pm$0.0913& 0.5940$\pm$0.1142& 0.4935$\pm$0.1450\\
3 & 0.7245$\pm$0.2434& 0.5738$\pm$0.1759& \textbf{0.4581}$\pm$0.1301& 0.8079$\pm$0.2838\\
5 & 0.9143$\pm$0.3235& 0.8422$\pm$0.2945& 0.9276$\pm$0.3208& \textbf{0.5265}$\pm$0.1611\\
7 & 0.9991$\pm$0.3505& 0.8267$\pm$0.2823& 1.0100$\pm$0.3554& \textbf{0.6161}$\pm$0.1986\\
9 & 1.0317$\pm$0.3707& 0.8139$\pm$0.2827& 0.8919$\pm$0.3072& \textbf{0.6466}$\pm$0.2054\\
\hline
\end{tabular}
}
\end{small}
\end{center}
\vspace{-20pt}
\end{table*}

% adv s9
% no attack\\
% 1\\
% 5\\
% 9\\


==> tables/table_exchange.tex <==
% \begin{table}[h]
% \caption{Metrics on exchange rate dataset under deterministic attack. No ground truth used in targeted attack.}
% \begin{center}
% \begin{small}
% \begin{tabular}{ccccccc}
% \hline
%  & \multicolumn{3}{c}{Relative norm} & \multicolumn{3}{c}{Targeted attack}\\
% \hline
% Sparsity & MAPE & MSE & wQL & MAPE & MSE & wQL\\
% \hline
% No attack & 0.0068 & 0.0001 & 0.0102  & 0.0096 & 0.0001 & 0.0112\\
% Enumerate & 0.0110 & 0.0002 & 0.0114  & 0.0074 & 0.0001 & 0.0107\\
% 1 & 0.0063 & 0.0001 & 0.0114 & 0.0061 & 0.0001 & 0.0112\\
% 3 & 0.0072 & 0.0001 & 0.0109 & 0.0078 & 0.0001 & 0.0100\\
% 5 & 0.0094 & 0.0001 & 0.0111 &  0.0089 & 0.0001 & 0.0106\\
% 7 & 0.0085 & 0.0001 & 0.0112 &  0.0086 & 0.0001 & 0.0105\\
% Full attack & 0.3482 & 0.1360 & 0.3323 & 0.3170 & 0.1303 & 0.2986\\
% \hline
% \end{tabular}
% \end{small}
% \end{center}
% \end{table}

\begin{table}[h]
\caption{Metrics on exchange rate dataset under deterministic attack. No ground truth used in targeted attack.}
\begin{center}
\begin{small}
\begin{tabular}{ccccccc}
\hline
 & \multicolumn{3}{c}{Targeted attack}\\
\hline
Sparsity & MAPE & MSE & wQL\\
\hline
no attack & 0.0065 & 0.0001 & 0.0101\\
enumerate & 0.0071 & 0.0001 & 0.0099\\
1 & 0.0065 & 0.0001 & 0.0102\\
3 & 0.0073 & 0.0001 & 0.0111\\
5 & 0.0068 & 0.0001 & 0.0111\\
7 & 0.0061 & 0.0001 & 0.0104\\
full attack & 0.3109 & 0.1253 & 0.2935\\
\hline
\end{tabular}
\end{small}
\end{center}
\end{table}

==> tables/table_exchange_sparse.tex <==
\begin{table}[h]
\caption{Metrics on exchange rate dataset under probabilistic attack using sparse layer. No ground truth used.}
\begin{center}
\begin{small}
\begin{tabular}{ccccccccc}
\hline
& \multicolumn{3}{c}{Using sparse Layer}\\
\hline
Sparsity & MAPE & MSE & wQL\\
\hline
no attack & 0.0088 & 0.0001 & 0.0109\\
1 & 0.0102 & 0.0002 & 0.0132\\
3 & 0.0151 & 0.0003 & 0.0124\\
5 & 0.0134 & 0.0002 & 0.0129\\
7 & 0.0174 & 0.0003 & 0.0151\\
\hline
\end{tabular}
\end{small}
\end{center}
\end{table}

==> tables/table_taxi.tex <==
\begin{table*}[h]
\caption{Metrics on taxi dataset under \textbf{deterministic} attack. Target time series $I=\{1\}$ and attacked time stamp $H=\{\tau\}$. Smaller is better.}
\label{table:taxi}
\begin{center}
\begin{small}
\scalebox{0.50}{
\begin{tabular}{ccccccccccccc}
\hline
 & \multicolumn{3}{c}{no defense} & \multicolumn{3}{c}{data augmentation} & \multicolumn{3}{c}{randomized smoothing} &\multicolumn{3}{c}{mini-max defense}\\
\hline
Sparsity & WAPE & WSE & wQL & WAPE & WSE & wQL & WAPE & WSE & wQL & WAPE & WSE & wQL\\
\hline
no attack & 3.1753$\pm$0.6548 & 16.3328$\pm$6.8222 & 1.2135$\pm$0.4050& 3.4020$\pm$0.6503 & 17.7390$\pm$7.2134 & 1.2137$\pm$0.4091& 3.4214$\pm$0.6501 & 17.8661$\pm$7.0561 & 1.2574$\pm$0.4281& 2.9366$\pm$0.6305 & 14.4184$\pm$6.3800 & \textbf{1.0447}$\pm$0.3607\\
1 & 3.2884$\pm$0.6591 & 17.1469$\pm$6.6485 & 1.3152$\pm$0.4580& 3.5884$\pm$0.6577 & 19.1832$\pm$7.1234 & 1.3455$\pm$0.4666& 3.6060$\pm$0.6559 & 19.2739$\pm$7.1416 & 1.3455$\pm$0.4627& 2.9776$\pm$0.6453 & 14.9359$\pm$6.4447 & \textbf{1.1222}$\pm$0.3960\\
3 & 3.8517$\pm$0.7110 & 22.2038$\pm$7.4880 & 1.6389$\pm$0.5810& 4.1630$\pm$0.7086 & 24.6490$\pm$8.2418 & 1.6805$\pm$0.5982& 4.1148$\pm$0.6872 & 23.8149$\pm$7.6266 & 1.6503$\pm$0.5756& 3.3441$\pm$0.6346 & 17.0547$\pm$6.1900 & \textbf{1.3624}$\pm$0.4956\\
5 & 4.5853$\pm$0.8062 & 30.5002$\pm$9.4037 & 2.0317$\pm$0.7161& 4.8419$\pm$0.7837 & 32.3970$\pm$9.5921 & 2.0625$\pm$0.7290& 4.7912$\pm$0.7643 & 31.4706$\pm$9.2416 & 2.0123$\pm$0.7059& 3.9484$\pm$0.6981 & 22.6945$\pm$7.6123 & \textbf{1.6830}$\pm$0.6206\\
7 & 5.2952$\pm$0.8884 & 39.5429$\pm$10.9774 & 2.3695$\pm$0.8064& 5.5116$\pm$0.9026 & 42.2533$\pm$11.8199 & 2.3712$\pm$0.8028& 5.3876$\pm$0.8831 & 40.3946$\pm$11.2429 & 2.3450$\pm$0.7978& 4.5162$\pm$0.8019 & 29.7695$\pm$9.1968 & \textbf{1.9750}$\pm$0.7033\\
9 & 5.7671$\pm$0.9517 & 46.4608$\pm$12.3892 & 2.5605$\pm$0.8531& 5.8631$\pm$0.9769 & 48.2877$\pm$13.5654 & 2.5525$\pm$0.8616& 5.8490$\pm$0.9610 & 47.6729$\pm$13.2402 & 2.5422$\pm$0.8619& 5.0564$\pm$0.8885 & 37.0739$\pm$10.9550 & \textbf{2.2374}$\pm$0.7785\\
full attack & 5.7407$\pm$0.9536 & 46.2118$\pm$12.1696 & 2.6222$\pm$0.8798& 5.7618$\pm$0.9307 & 45.8250$\pm$12.4133 & 2.5579$\pm$0.8795& 5.6389$\pm$0.9092 & 43.8469$\pm$11.5653 & 2.5403$\pm$0.8761& 4.4621$\pm$0.8612 & 30.7219$\pm$9.7170 & \textbf{2.0377}$\pm$0.7526\\
\hline
\end{tabular}
}
\end{small}
\end{center}
\end{table*}



==> tables/table_taxi_new.tex <==
\begin{table*}[h]
\caption{Average wQL on electricity dataset under \textbf{deterministic} and \textbf{probabilistic} attack. Target time series $I=\{1\}$ and attacked time stamp $H=\{\tau\}$. Smaller is better.}
\label{table:taxi_new}
\begin{center}
\begin{small}
\scalebox{1}{
\begin{tabular}{c|cccc|cccc}
\hline
 & \multicolumn{4}{c|}{deterministic attack} & \multicolumn{4}{c}{probabilistic attack}\\
\hline
Sparsity & no defense & DA & RS & mini-max & no defense & DA & RS & mini-max\\
\hline
no attack & 1.2135& 1.2137& 1.2574& \textbf{1.0447} & 1.2135& 1.2137& 1.2574& \textbf{1.0447}\\
1 & 1.3152& 1.3455& 1.3455& \textbf{1.1222}& 1.4598& 1.3539& 1.3512& \textbf{1.1528}\\
3 & 1.6389& 1.6805& 1.6503& \textbf{1.3624}& 1.5659& 1.5446& 1.5567& \textbf{1.3940}\\
5 & 2.0317& 2.0625& 2.0123& \textbf{1.6830}& 1.9123& 1.7824& 1.8857& \textbf{1.6897}\\
7 & 2.3695& 2.3712& 2.3450& \textbf{1.9750}& 2.2915& 1.7340& 1.8370& \textbf{1.5865}\\
9 & 2.5605& 2.5525& 2.5422& \textbf{2.2374} & 2.4815& 2.1159& 2.2400& \textbf{1.4921}\\
\hline
\end{tabular}
}
\end{small}
\end{center}
\end{table*}


==> tables/table_taxi_sparse.tex <==
\begin{table*}[h]
\caption{Metrics on taxi dataset under \textbf{probabilistic} attack.  Target time series $I=\{1\}$ and attacked time stamp $H=\{\tau\}$. Smaller is better.}
\label{table:taxi_sparse}
\begin{center}
\begin{small}
\scalebox{0.50}{
\begin{tabular}{ccccccccccccc}
\hline
 & \multicolumn{3}{c}{no defense} & \multicolumn{3}{c}{data augmentation} & \multicolumn{3}{c}{randomized smoothing} &\multicolumn{3}{c}{mini-max defense}\\
\hline
Sparsity & WAPE & WSE & wQL & WAPE & WSE & wQL & WAPE & WSE & wQL & WAPE & WSE & wQL\\
\hline
no attack & 3.2019$\pm$0.6620 & 16.6407$\pm$7.0108 & 1.2118$\pm$0.4412& 3.4348$\pm$0.6568 & 18.0856$\pm$7.3327 & 1.2526$\pm$0.4733& 3.3940$\pm$0.6477 & 17.6348$\pm$7.0878 & 1.2241$\pm$0.4531& 2.9964$\pm$0.6383 & 14.9179$\pm$6.7198 & \textbf{1.0481}$\pm$0.3840\\
1 & 3.5098$\pm$0.7117 & 19.7020$\pm$7.1520 & 1.4598$\pm$0.5315& 3.5353$\pm$0.6450 & 18.5629$\pm$6.7227 & 1.3539$\pm$0.5199& 3.5961$\pm$0.6397 & 18.8968$\pm$6.6969 & 1.3512$\pm$0.5100& 3.0503$\pm$0.6183 & 14.8761$\pm$6.0088 & \textbf{1.1528}$\pm$0.4345\\
3 & 3.5043$\pm$0.7429 & 20.3267$\pm$8.1305 & 1.5659$\pm$0.6589& 3.7547$\pm$0.7278 & 21.8185$\pm$7.6430 & 1.5446$\pm$0.6197& 3.8490$\pm$0.7015 & 21.9873$\pm$7.0132 & 1.5567$\pm$0.5784& 2.9650$\pm$0.6868 & 15.6679$\pm$6.3028 & \textbf{1.3940}$\pm$0.5472\\
5 & 4.2285$\pm$0.7365 & 25.7872$\pm$7.6545 & 1.9123$\pm$0.7513& 3.9991$\pm$0.7031 & 23.1989$\pm$6.9567 & 1.7824$\pm$0.6962& 4.1910$\pm$0.7303 & 25.3399$\pm$7.4696 & 1.8857$\pm$0.7441& 2.9543$\pm$0.5872 & 13.7538$\pm$4.4577 & \textbf{1.6897}$\pm$0.6829\\
7 & 4.7813$\pm$0.8095 & 32.4134$\pm$9.1638 & 2.2915$\pm$0.8954& 3.8031$\pm$0.7747 & 23.2123$\pm$8.9699 & 1.7340$\pm$0.7638& 4.3014$\pm$0.7394 & 26.4713$\pm$9.5438 & 1.8370$\pm$0.7597& 3.1284$\pm$0.7122 & 17.1805$\pm$6.8163 & \textbf{1.5865}$\pm$0.6191\\
9 & 5.3666$\pm$0.8732 & 39.9142$\pm$10.3507 & 2.4815$\pm$0.9286& 5.0260$\pm$0.7627 & 33.7399$\pm$8.1455 & 2.1159$\pm$0.7515& 5.3652$\pm$0.8100 & 38.3500$\pm$9.4049 & 2.2400$\pm$0.7860& 3.1476$\pm$0.6961 & 16.9713$\pm$6.2469 & \textbf{1.4921}$\pm$0.5551\\
\hline
\end{tabular}
}
\end{small}
\end{center}
\end{table*}

% s5 adv

==> tables/table_traffic.tex <==
\begin{table*}[h]
\caption{Metrics on traffic dataset under \textbf{deterministic} attack. No ground truth used in targeted attack.}
\begin{center}
\begin{small}
\scalebox{0.5}{
\begin{tabular}{ccccccccccccc}
\hline
 & \multicolumn{3}{c}{no defense} & \multicolumn{3}{c}{data augmentation} & \multicolumn{3}{c}{randomized smoothing} &\multicolumn{3}{c}{mini-max defense}\\
\hline
Sparsity & MAPE & MSE & wQL & MAPE & MSE & wQL & MAPE & MSE & wQL & MAPE & MSE & wQL\\
\hline
% no attack & 0.2296 & 0.0812 & 0.2029 & 0.2297 & 0.0905 & 0.2004 & 0.2244 & 0.0910 & \textbf{0.1925} & 0.4452 & 0.2272 & 0.3517\\
% 1 & 0.2360 & 0.0894 & 0.2099 & 0.2753 & 0.1049 & 0.2184 & 0.2470 & 0.0878 & \textbf{0.1986} & 0.4891 & 0.2635 & 0.3816\\
% 5 & 0.4634 & 0.2916 & 0.3170 & 0.6823 & 0.8220 & 0.5124 & 0.6293 & 0.6541 & 0.4809 & 0.3610 & 0.1755 & \textbf{0.3071}\\
% 9 & 0.8491 & 1.0602 & 0.5936 & 1.1590 & 1.7384 & 0.8535 & 1.0774 & 1.5025 & 0.8025 & 0.2875 & 0.1116 & \textbf{0.3068}\\
% full attack & 1.0149 & 1.3282 & 0.6918 & 1.4463 & 2.3638 & 1.0210 & 1.3594 & 2.1308 & 0.9973 & 0.3150 & 0.1127 & \textbf{0.5643}\\
% no attack & 0.2301 & 0.0797 & 0.2024& 0.2347 & 0.0924 & 0.2026& 0.2317 & 0.0959 & 0.2031& 0.7036 & 0.5298 & 0.4905\\
% 1 & 0.2540 & 0.1039 & 0.2169& 0.2658 & 0.1305 & 0.2288& 0.2592 & 0.1201 & 0.2205& 0.7037 & 0.5064 & 0.4933\\
% 3 & 0.2690 & 0.1167 & 0.2192& 0.3840 & 0.2253 & 0.2779& 0.3510 & 0.1557 & 0.2559& 0.6246 & 0.4002 & 0.4499\\
% 5 & 0.4389 & 0.2897 & 0.3200& 0.5388 & 0.4552 & 0.4078& 0.5295 & 0.4354 & 0.3851& 0.5828 & 0.3590 & 0.4262\\
% 7 & 0.5862 & 0.4795 & 0.4019& 0.6772 & 0.7989 & 0.5138& 0.6271 & 0.6205 & 0.4723& 0.5038 & 0.2765 & 0.3870\\
% 9 & 0.6932 & 0.7399 & 0.5030& 0.7626 & 0.9388 & 0.5947& 0.7802 & 0.9588 & 0.6120& 0.5063 & 0.2938 & 0.3954\\
% full attack & 0.8048 & 0.9935 & 0.6263& 0.8637 & 1.0820 & 0.6417& 0.7954 & 0.8799 & 0.5884& 0.4999 & 0.2978 & 0.3873\\
% no attack & 0.2777$\pm$0.1533 & 0.1006$\pm$0.0856 & 0.2211$\pm$0.1745& 0.2393$\pm$0.1795 & 0.0895$\pm$0.0888 & \textbf{0.1922}$\pm$0.1643& 0.2300$\pm$0.1803 & 0.0854$\pm$0.0893 & 0.1982$\pm$0.1704& 0.2498$\pm$0.1537 & 0.0860$\pm$0.1010 & 0.2158$\pm$0.1920\\
% 1 & 0.3012$\pm$0.1772 & 0.1221$\pm$0.1087 & 0.2350$\pm$0.1755& 0.2438$\pm$0.1729 & 0.0893$\pm$0.0968 & 0.1942$\pm$0.1621& 0.2482$\pm$0.1730 & 0.0916$\pm$0.0927 & 0.1991$\pm$0.1592& 0.2227$\pm$0.1467 & 0.0711$\pm$0.0891 & \textbf{0.1834}$\pm$0.1732\\
% 3 & 0.3126$\pm$0.2187 & 0.1455$\pm$0.1428 & 0.2494$\pm$0.2077& 0.2992$\pm$0.1614 & 0.1156$\pm$0.1255 & 0.2155$\pm$0.1513& 0.2970$\pm$0.1910 & 0.1247$\pm$0.1334 & 0.2197$\pm$0.1693& 0.2110$\pm$0.1522 & 0.0677$\pm$0.0894 & \textbf{0.1741}$\pm$0.1745\\
% 5 & 0.3869$\pm$0.2333 & 0.2041$\pm$0.1869 & 0.2938$\pm$0.2328& 0.3827$\pm$0.2435 & 0.2058$\pm$0.2192 & 0.2671$\pm$0.2218& 0.3549$\pm$0.2223 & 0.1754$\pm$0.1880 & 0.2529$\pm$0.2061& 0.1836$\pm$0.1524 & 0.0569$\pm$0.0817 & \textbf{0.1479}$\pm$0.1646\\
% 7 & 0.5003$\pm$0.3286 & 0.3582$\pm$0.4239 & 0.3691$\pm$0.3131& 0.4816$\pm$0.3197 & 0.3341$\pm$0.3312 & 0.3486$\pm$0.2718& 0.4786$\pm$0.3053 & 0.3222$\pm$0.3261 & 0.3406$\pm$0.2618& 0.2038$\pm$0.1718 & 0.0711$\pm$0.0928 & \textbf{0.1569}$\pm$0.1632\\
% 9 & 0.5877$\pm$0.3861 & 0.4945$\pm$0.5468 & 0.4257$\pm$0.3641& 0.6140$\pm$0.4260 & 0.5585$\pm$0.6076 & 0.4519$\pm$0.3809& 0.6316$\pm$0.3923 & 0.5528$\pm$0.5504 & 0.4515$\pm$0.3632& 0.2324$\pm$0.2439 & 0.1135$\pm$0.1815 & \textbf{0.1942}$\pm$0.2111\\
% full attack & 0.8157$\pm$0.5179 & 0.9335$\pm$0.9884 & 0.6078$\pm$0.4616& 0.8615$\pm$0.4742 & 0.9671$\pm$0.8805 & 0.6167$\pm$0.4362& 0.8394$\pm$0.4589 & 0.9153$\pm$0.8358 & 0.5908$\pm$0.4397& 0.3005$\pm$0.2467 & 0.1512$\pm$0.2181 & \textbf{0.2256}$\pm$0.1983\\
no attack & 0.2591$\pm$0.1002 & 0.0854$\pm$0.0494 & 0.2109$\pm$0.0941& 0.1651$\pm$0.1319 & 0.0590$\pm$0.0552 & 0.1539$\pm$0.0997& 0.1773$\pm$0.1341 & 0.0642$\pm$0.0639 & 0.1595$\pm$0.1043& 0.2539$\pm$0.0891 & 0.0789$\pm$0.0573 & 0.1977$\pm$0.0878\\
1 & 0.2557$\pm$0.1046 & 0.0853$\pm$0.0493 & 0.2066$\pm$0.0899& 0.1732$\pm$0.1142 & 0.0538$\pm$0.0507 & 0.1433$\pm$0.0866& 0.1689$\pm$0.1124 & 0.0515$\pm$0.0484 & 0.1397$\pm$0.0819& 0.2360$\pm$0.1007 & 0.0742$\pm$0.0610 & 0.1878$\pm$0.0905\\
3 & 0.3319$\pm$0.1656 & 0.1602$\pm$0.1163 & 0.2656$\pm$0.1346& 0.2334$\pm$0.1403 & 0.0903$\pm$0.0864 & 0.1723$\pm$0.0929& 0.2535$\pm$0.1309 & 0.0955$\pm$0.0801 & 0.1936$\pm$0.0940& 0.1947$\pm$0.1204 & 0.0643$\pm$0.0608 & 0.1551$\pm$0.0869\\
5 & 0.4122$\pm$0.2279 & 0.2646$\pm$0.2112 & 0.3132$\pm$0.1779& 0.3972$\pm$0.2361 & 0.2593$\pm$0.2657 & 0.2780$\pm$0.1553& 0.3949$\pm$0.2237 & 0.2471$\pm$0.2517 & 0.2827$\pm$0.1522& 0.1933$\pm$0.1428 & 0.0745$\pm$0.0739 & 0.1645$\pm$0.0911\\
7 & 0.4805$\pm$0.2488 & 0.3437$\pm$0.2792 & 0.3597$\pm$0.2067& 0.5899$\pm$0.2697 & 0.4805$\pm$0.4418 & 0.3901$\pm$0.1741& 0.5427$\pm$0.2867 & 0.4443$\pm$0.4656 & 0.3678$\pm$0.1904& 0.2736$\pm$0.1815 & 0.1349$\pm$0.1440 & 0.2105$\pm$0.1225\\
9 & 0.6040$\pm$0.2886 & 0.5165$\pm$0.3653 & 0.4607$\pm$0.2290& 0.6354$\pm$0.2575 & 0.5245$\pm$0.3475 & 0.4453$\pm$0.1461& 0.7024$\pm$0.3376 & 0.7011$\pm$0.6320 & 0.5006$\pm$0.2223& 0.3074$\pm$0.1750 & 0.1503$\pm$0.1600 & 0.2243$\pm$0.1349\\
full attack & 0.7321$\pm$0.3497 & 0.7587$\pm$0.5301 & 0.5492$\pm$0.2677& 0.7590$\pm$0.3224 & 0.7654$\pm$0.4715 & 0.5339$\pm$0.2018& 0.7424$\pm$0.2922 & 0.7069$\pm$0.4756 & 0.5273$\pm$0.2046& 0.3742$\pm$0.1725 & 0.1942$\pm$0.1743 & 0.2611$\pm$0.1242\\
\hline
\end{tabular}
}
\end{small}
\end{center}
\end{table*}




% mini-max + rs
% no attack & 0.4422 & 0.2336 & 0.3656\\
% 1 & 0.4692 & 0.2470 & 0.3651\\
% 5 & 0.3877 & 0.2000 & 0.3289\\
% 9 & 0.3359 & 0.1447 & 0.3226\\
% full attack & 0.2978 & 0.1104 & 0.3432\\


==> tables/table_traffic_comp.tex <==

\begin{table*}[h]
\caption{Metrics on traffic dataset under \textbf{deterministic} attack. Target time series $I=\{1, 5\}$ and attacked time stamp $H=\{\tau-1, \tau\}$. Smaller is better.}
\begin{center}
\begin{small}
\scalebox{0.5}{
\begin{tabular}{ccccccccccccc}
\hline
 & \multicolumn{3}{c}{no defense} & \multicolumn{3}{c}{data augmentation} & \multicolumn{3}{c}{randomized smoothing} &\multicolumn{3}{c}{mini-max defense}\\
\hline
Sparsity & MAPE & MSE & wQL & MAPE & MSE & wQL & MAPE & MSE & wQL & MAPE & MSE & wQL\\
\hline
no attack & 0.3241$\pm$0.1961 & 0.1751$\pm$0.2128 & 0.2283$\pm$0.0838& 0.2334$\pm$0.1358 & 0.0881$\pm$0.0854 & 0.1573$\pm$0.0609& 0.2237$\pm$0.1398 & 0.0857$\pm$0.1007 & 0.1529$\pm$0.0628& 0.2619$\pm$0.0970 & 0.0857$\pm$0.0608 & 0.1837$\pm$0.0551\\
1 & 0.3169$\pm$0.1687 & 0.1522$\pm$0.1474 & 0.2190$\pm$0.0816& 0.2311$\pm$0.1355 & 0.0869$\pm$0.0926 & 0.1543$\pm$0.0537& 0.2328$\pm$0.1321 & 0.0860$\pm$0.0903 & 0.1529$\pm$0.0484& 0.2628$\pm$0.1178 & 0.0944$\pm$0.0762 & 0.1701$\pm$0.0528\\
3 & 0.3161$\pm$0.1563 & 0.1445$\pm$0.1288 & 0.2150$\pm$0.0845& 0.3098$\pm$0.1483 & 0.1361$\pm$0.1282 & 0.1884$\pm$0.0495& 0.3094$\pm$0.1405 & 0.1317$\pm$0.1130 & 0.1890$\pm$0.0449& 0.2789$\pm$0.1382 & 0.1126$\pm$0.1010 & 0.1687$\pm$0.0507\\
5 & 0.4199$\pm$0.2101 & 0.2568$\pm$0.2098 & 0.2772$\pm$0.1138& 0.4547$\pm$0.2155 & 0.2914$\pm$0.2922 & 0.2729$\pm$0.0822& 0.4579$\pm$0.2172 & 0.2956$\pm$0.2956 & 0.2648$\pm$0.0741& 0.3053$\pm$0.1675 & 0.1444$\pm$0.1337 & 0.1688$\pm$0.0399\\
7 & 0.5273$\pm$0.2538 & 0.3953$\pm$0.2984 & 0.3620$\pm$0.1398& 0.5693$\pm$0.2393 & 0.4284$\pm$0.3438 & 0.3597$\pm$0.0852& 0.5684$\pm$0.2627 & 0.4489$\pm$0.4206 & 0.3535$\pm$0.1006& 0.3303$\pm$0.1877 & 0.1733$\pm$0.1618 & 0.1779$\pm$0.0474\\
9 & 0.7067$\pm$0.2875 & 0.6501$\pm$0.4078 & 0.4635$\pm$0.1431& 0.6294$\pm$0.2545 & 0.5142$\pm$0.3943 & 0.4058$\pm$0.0885& 0.6493$\pm$0.2493 & 0.5348$\pm$0.3959 & 0.4240$\pm$0.0743& 0.3794$\pm$0.2202 & 0.2323$\pm$0.2076 & 0.1970$\pm$0.0395\\
full attack & 0.9268$\pm$0.4233 & 1.1855$\pm$0.8775 & 0.5714$\pm$0.1726& 0.6837$\pm$0.2451 & 0.5770$\pm$0.3648 & 0.4687$\pm$0.1061& 0.7221$\pm$0.2552 & 0.6401$\pm$0.4089 & 0.4820$\pm$0.1030& 0.4542$\pm$0.2111 & 0.2875$\pm$0.2133 & 0.2634$\pm$0.0812\\
\hline
\end{tabular}
}
\end{small}
\end{center}
\end{table*}



==> tables/table_traffic_comp_short.tex <==
\begin{table*}[h]
\caption{Average wQL on Traffic dataset under \textbf{deterministic} attack. Target time series $I=\{1, 5\}$ and attacked time stamp $H=\{\tau-1, \tau\}$. Smaller is better.}
\label{table:traffic_short}
\begin{center}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{ccccccccccccc}
\hline
Sparsity & no defense & data augmentation & randomized smoothing & mini-max defense\\
\hline
no attack & 0.2283$\pm$0.0838& 0.1573$\pm$0.0609& \textbf{0.1529}$\pm$0.0628& 0.1837$\pm$0.0551\\
1 & 0.2190$\pm$0.0816& 0.1543$\pm$0.0537& \textbf{0.1529}$\pm$0.0484& 0.1701$\pm$0.0528\\
3 & 0.2150$\pm$0.0845& 0.1884$\pm$0.0495& 0.1890$\pm$0.0449& \textbf{0.1687}$\pm$0.0507\\
5 & 0.2772$\pm$0.1138& 0.2729$\pm$0.0822& 0.2648$\pm$0.0741& \textbf{0.1688}$\pm$0.0399\\
7 & 0.3620$\pm$0.1398& 0.3597$\pm$0.0852& 0.3535$\pm$0.1006& \textbf{0.1779}$\pm$0.0474\\
9 & 0.4635$\pm$0.1431& 0.4058$\pm$0.0885& 0.4240$\pm$0.0743& \textbf{0.1970}$\pm$0.0395\\
\hline
\end{tabular}
}
\end{small}
\end{center}
\end{table*}


==> tables/table_traffic_short.tex <==
\begin{table*}[h]
\caption{Average wQL on Traffic dataset under \textbf{deterministic} attack. Target time series $I=\{1\}$ and attacked time stamp $H=\{\tau\}$. Smaller is better.}
\label{table:traffic_short}
\begin{center}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{ccccccccccccc}
\hline
Sparsity & no defense & data augmentation & randomized smoothing & mini-max defense\\
\hline
no attack & 0.2109$\pm$0.0941& \textbf{0.1539}$\pm$0.0997& 0.1595$\pm$0.1043& 0.1977$\pm$0.0878\\
1 & 0.2066$\pm$0.0899& 0.1433$\pm$0.0866& \textbf{0.1397}$\pm$0.0819& 0.1878$\pm$0.0905\\
3 & 0.2656$\pm$0.1346& 0.1723$\pm$0.0929& 0.1936$\pm$0.0940& \textbf{0.1551}$\pm$0.0869\\
5 & 0.3132$\pm$0.1779& 0.2780$\pm$0.1553& 0.2827$\pm$0.1522& \textbf{0.1645}$\pm$0.0911\\
7 & 0.3597$\pm$0.2067& 0.3901$\pm$0.1741& 0.3678$\pm$0.1904& \textbf{0.2105}$\pm$0.1225\\
9 & 0.4607$\pm$0.2290& 0.4453$\pm$0.1461& 0.5006$\pm$0.2223& \textbf{0.2243}$\pm$0.1349\\
full attack & 0.5492$\pm$0.2677& 0.5339$\pm$0.2018& 0.5273$\pm$0.2046& \textbf{0.2611}$\pm$0.1242\\
\hline
\end{tabular}
}
\end{small}
\end{center}
\end{table*}


==> tables/table_traffic_sparse.tex <==
\begin{table}[h]
\caption{Metrics on traffic dataset under \textbf{probabilistic} attack. Target time series $I=\{1\}$ and attacked time stamp $H=\{\tau\}$. Smaller is better.}
\begin{center}
\begin{small}
\scalebox{0.5}{
\begin{tabular}{ccccccccccccc}
\hline
 & \multicolumn{3}{c}{no defense} & \multicolumn{3}{c}{data augmentation} & \multicolumn{3}{c}{randomized smoothing} &\multicolumn{3}{c}{mini-max defense}\\
\hline
Sparsity & MAPE & MSE & wQL & MAPE & MSE & wQL & MAPE & MSE & wQL & MAPE & MSE & wQL\\
\hline
no attack & 0.2784$\pm$0.1142 & 0.1013$\pm$0.0623 & 0.2248$\pm$0.1259& 0.1727$\pm$0.1270 & 0.0592$\pm$0.0565 & 0.1510$\pm$0.1156& 0.1728$\pm$0.1272 & 0.0593$\pm$0.0568 & 0.1515$\pm$0.1116& 0.2354$\pm$0.0929 & 0.0711$\pm$0.0572 & 0.1867$\pm$0.1137\\
1 & 0.2674$\pm$0.1542 & 0.1148$\pm$0.1025 & 0.2185$\pm$0.1640& 0.2344$\pm$0.1445 & 0.0930$\pm$0.0926 & 0.1921$\pm$0.1391& 0.2367$\pm$0.1428 & 0.0932$\pm$0.0911 & 0.1902$\pm$0.1301& 0.2632$\pm$0.1012 & 0.0879$\pm$0.0639 & 0.2044$\pm$0.1165\\
3 & 0.3469$\pm$0.1937 & 0.1887$\pm$0.1583 & 0.2745$\pm$0.1760& 0.2613$\pm$0.2046 & 0.1446$\pm$0.1767 & 0.2141$\pm$0.1743& 0.2724$\pm$0.2024 & 0.1488$\pm$0.1851 & 0.2172$\pm$0.1791& 0.2336$\pm$0.1181 & 0.0800$\pm$0.0667 & 0.1888$\pm$0.1198\\
5 & 0.4215$\pm$0.2269 & 0.2714$\pm$0.2673 & 0.3232$\pm$0.2189& 0.4222$\pm$0.2222 & 0.2682$\pm$0.2925 & 0.2957$\pm$0.2076& 0.4160$\pm$0.2028 & 0.2480$\pm$0.2577 & 0.2838$\pm$0.1826& 0.1966$\pm$0.1203 & 0.0650$\pm$0.0609 & 0.1620$\pm$0.1046\\
7 & 0.6423$\pm$0.3099 & 0.5875$\pm$0.4923 & 0.4618$\pm$0.2937& 0.5302$\pm$0.3097 & 0.4558$\pm$0.5056 & 0.3634$\pm$0.2531& 0.5438$\pm$0.3131 & 0.4744$\pm$0.5129 & 0.3775$\pm$0.2630& 0.2529$\pm$0.1650 & 0.1136$\pm$0.1054 & 0.1983$\pm$0.1196\\
9 & 0.6232$\pm$0.2960 & 0.5481$\pm$0.4104 & 0.4539$\pm$0.2693& 0.7473$\pm$0.4367 & 0.9060$\pm$0.9633 & 0.5342$\pm$0.3896& 0.6902$\pm$0.3470 & 0.6958$\pm$0.6304 & 0.4707$\pm$0.2950& 0.3203$\pm$0.1795 & 0.1613$\pm$0.1607 & 0.2352$\pm$0.1464\\
\hline
\end{tabular}
}
\end{small}
\end{center}
\end{table}


==> tables/table_traffic_sparse_comp.tex <==

\begin{table}[h]
\caption{Metrics on traffic dataset under \textbf{probabilistic} attack. Target time series $I=\{1,5\}$ and attacked time stamp $H=\{\tau-1, \tau\}$. Smaller is better.}
\begin{center}
\begin{small}
\scalebox{0.5}{
\begin{tabular}{ccccccccccccc}
\hline
 & \multicolumn{3}{c}{no defense} & \multicolumn{3}{c}{data augmentation} & \multicolumn{3}{c}{randomized smoothing} &\multicolumn{3}{c}{mini-max defense}\\
\hline
Sparsity & MAPE & MSE & wQL & MAPE & MSE & wQL & MAPE & MSE & wQL & MAPE & MSE & wQL\\
\hline
no attack & 0.3247$\pm$0.1935 & 0.1736$\pm$0.2082 & 0.2283$\pm$0.1015& 0.2259$\pm$0.1332 & 0.0833$\pm$0.0916 & 0.1547$\pm$0.0719& 0.2307$\pm$0.1381 & 0.0879$\pm$0.0912 & 0.1575$\pm$0.0739& 0.2710$\pm$0.1114 & 0.0960$\pm$0.0766 & 0.1820$\pm$0.0762\\
1 & 0.3407$\pm$0.1987 & 0.1881$\pm$0.2304 & 0.2428$\pm$0.1191& 0.2514$\pm$0.1554 & 0.1072$\pm$0.1096 & 0.1807$\pm$0.1009& 0.2502$\pm$0.1535 & 0.1055$\pm$0.1106 & 0.1796$\pm$0.0990& 0.2777$\pm$0.1072 & 0.0981$\pm$0.0749 & 0.1904$\pm$0.0734\\
3 & 0.3152$\pm$0.1863 & 0.1626$\pm$0.1879 & 0.2219$\pm$0.1271& 0.3525$\pm$0.2043 & 0.2003$\pm$0.1880 & 0.2564$\pm$0.1372& 0.3522$\pm$0.2037 & 0.1997$\pm$0.1831 & 0.2467$\pm$0.1235& 0.2749$\pm$0.1309 & 0.1068$\pm$0.0898 & 0.1714$\pm$0.0709\\
5 & 0.4230$\pm$0.2683 & 0.3101$\pm$0.3357 & 0.2719$\pm$0.1451& 0.4537$\pm$0.1674 & 0.2569$\pm$0.1773 & 0.3026$\pm$0.1223& 0.4573$\pm$0.1635 & 0.2578$\pm$0.1680 & 0.3003$\pm$0.1261& 0.2981$\pm$0.1404 & 0.1248$\pm$0.0974 & 0.1883$\pm$0.0781\\
7 & 0.5214$\pm$0.2692 & 0.4038$\pm$0.3264 & 0.3529$\pm$0.1707& 0.4383$\pm$0.2126 & 0.2745$\pm$0.2613 & 0.2893$\pm$0.1379& 0.4473$\pm$0.2183 & 0.2870$\pm$0.2684 & 0.2824$\pm$0.1339& 0.3017$\pm$0.1530 & 0.1337$\pm$0.1049 & 0.1846$\pm$0.0751\\
9 & 0.6694$\pm$0.2931 & 0.6047$\pm$0.4627 & 0.4075$\pm$0.1550& 0.5242$\pm$0.2466 & 0.3857$\pm$0.2916 & 0.3544$\pm$0.1460& 0.5147$\pm$0.2383 & 0.3684$\pm$0.2919 & 0.3376$\pm$0.1406& 0.2866$\pm$0.1563 & 0.1266$\pm$0.1116 & 0.1911$\pm$0.0843\\
\hline
\end{tabular}
}
\end{small}
\end{center}
\end{table}


==> tables/table_traffic_sparse_comp_short.tex <==
\begin{table*}[h]
\caption{Average wQL on Traffic dataset under \textbf{probabilistic} attack. Target time series $I=\{1,5\}$ and attacked time stamp $H=\{\tau-1,\tau\}$. Smaller is better.}
\label{table:traffic_sparse_short}
\begin{center}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{ccccccccccccc}
\hline
Sparsity & no defense & data augmentation & randomized smoothing & mini-max defense\\
\hline
no attack & 0.2283$\pm$0.1015& \textbf{0.1547}$\pm$0.0719& 0.1575$\pm$0.0739& 0.1820$\pm$0.0762\\
1 & 0.2428$\pm$0.1191& 0.1807$\pm$0.1009& \textbf{0.1796}$\pm$0.0990& 0.1904$\pm$0.0734\\
3 & 0.2219$\pm$0.1271& 0.2564$\pm$0.1372& 0.2467$\pm$0.1235& \textbf{0.1714}$\pm$0.0709\\
5 & 0.2719$\pm$0.1451& 0.3026$\pm$0.1223& 0.3003$\pm$0.1261& \textbf{0.1883}$\pm$0.0781\\
7 & 0.3529$\pm$0.1707& 0.2893$\pm$0.1379& 0.2824$\pm$0.1339& \textbf{0.1846}$\pm$0.0751\\
9 & 0.4075$\pm$0.1550& 0.3544$\pm$0.1460& 0.3376$\pm$0.1406& \textbf{0.1911}$\pm$0.0843\\
\hline
\end{tabular}
}
\end{small}
\end{center}
\end{table*}


==> tables/table_traffic_sparse_short.tex <==
\begin{table*}[h]
\caption{Average wQL on Traffic dataset under \textbf{probabilistic} attack. Target time series $I=\{1\}$ and attacked time stamp $H=\{\tau\}$. Smaller is better.}
\label{table:electricity}
\begin{center}
\begin{small}
\scalebox{0.8}{
\begin{tabular}{ccccccccccccc}
\hline
Sparsity & no defense & data augmentation & randomized smoothing & mini-max defense\\
\hline
no attack & 0.2248$\pm$0.1259& \textbf{0.1510}$\pm$0.1156& 0.1515$\pm$0.1116& 0.1867$\pm$0.1137\\
1 & 0.2185$\pm$0.1640& 0.1921$\pm$0.1391& \textbf{0.1902}$\pm$0.1301& 0.2044$\pm$0.1165\\
3 & 0.2745$\pm$0.1760& 0.2141$\pm$0.1743& 0.2172$\pm$0.1791& \textbf{0.1888}$\pm$0.1198\\
5 & 0.3232$\pm$0.2189& 0.2957$\pm$0.2076& 0.2838$\pm$0.1826& \textbf{0.1620}$\pm$0.1046\\
7 & 0.4618$\pm$0.2937& 0.3634$\pm$0.2531& 0.3775$\pm$0.2630& \textbf{0.1983}$\pm$0.1196\\
9 & 0.4539$\pm$0.2693& 0.5342$\pm$0.3896& 0.4707$\pm$0.2950& \textbf{0.2352}$\pm$0.1464\\
\hline
\end{tabular}
}
\end{small}
\end{center}
\end{table*}


==> tables/table_wiki.tex <==
\begin{table*}[h]
\caption{Metrics on Wiki dataset under \textbf{deterministic} attack. No ground truth used in targeted attack.}
\begin{center}
\begin{small}
\scalebox{0.5}{
\begin{tabular}{ccccccccccccc}
\hline
 & \multicolumn{3}{c}{no defense} & \multicolumn{3}{c}{data augmentation} & \multicolumn{3}{c}{randomized smoothing} &\multicolumn{3}{c}{mini-max defense}\\
\hline
Sparsity & MAPE & MSE & wQL & MAPE & MSE & wQL & MAPE & MSE & wQL & MAPE & MSE & wQL\\
\hline
no attack & 0.2697$\pm$0.1367 & 0.0971$\pm$0.0744 & 0.1645$\pm$0.0588& 0.0962$\pm$0.0569 & 0.0135$\pm$0.0116 & 0.0868$\pm$0.0232& 0.0982$\pm$0.0535 & 0.0134$\pm$0.0122 & 0.0796$\pm$0.0272& 0.2599$\pm$0.1431 & 0.0942$\pm$0.0669 & 0.2331$\pm$0.1186\\
1 & 0.3948$\pm$0.1357 & 0.1798$\pm$0.1010 & 0.2430$\pm$0.0889& 0.0963$\pm$0.0469 & 0.0121$\pm$0.0100 & 0.0775$\pm$0.0171& 0.0783$\pm$0.0474 & 0.0091$\pm$0.0075 & 0.0687$\pm$0.0119& 0.1960$\pm$0.1277 & 0.0597$\pm$0.0664 & 0.1683$\pm$0.1097\\
3 & 0.4706$\pm$0.1256 & 0.2420$\pm$0.1400 & 0.2771$\pm$0.0807& 0.3138$\pm$0.1756 & 0.1386$\pm$0.1149 & 0.2225$\pm$0.1217& 0.3180$\pm$0.1574 & 0.1334$\pm$0.1001 & 0.2260$\pm$0.1089& 0.1937$\pm$0.1163 & 0.0551$\pm$0.0555 & 0.1466$\pm$0.0976\\
5 & 0.6571$\pm$0.1439 & 0.4587$\pm$0.2007 & 0.4260$\pm$0.1127& 0.4849$\pm$0.1890 & 0.2817$\pm$0.1983 & 0.3533$\pm$0.1602& 0.4406$\pm$0.1651 & 0.2296$\pm$0.1576 & 0.3084$\pm$0.1365& 0.2376$\pm$0.1145 & 0.0735$\pm$0.0462 & 0.1675$\pm$0.0675\\
7 & 0.7477$\pm$0.1169 & 0.5768$\pm$0.1940 & 0.5173$\pm$0.1045& 0.5884$\pm$0.1840 & 0.3903$\pm$0.2277 & 0.4290$\pm$0.1524& 0.5662$\pm$0.1710 & 0.3586$\pm$0.2184 & 0.4112$\pm$0.1420& 0.3094$\pm$0.0983 & 0.1083$\pm$0.0670 & 0.1973$\pm$0.0632\\
9 & 0.8458$\pm$0.1400 & 0.7409$\pm$0.2442 & 0.6276$\pm$0.1178& 0.5937$\pm$0.1602 & 0.3859$\pm$0.2071 & 0.4362$\pm$0.1360& 0.6020$\pm$0.1718 & 0.4009$\pm$0.2340 & 0.4451$\pm$0.1461& 0.3175$\pm$0.1501 & 0.1301$\pm$0.1063 & 0.2185$\pm$0.1131\\
full attack & 1.6039$\pm$0.2748 & 2.6708$\pm$0.9348 & 1.2957$\pm$0.2168& 0.1778$\pm$0.1007 & 0.0448$\pm$0.0399 & 0.1518$\pm$0.0781& 0.1727$\pm$0.1082 & 0.0450$\pm$0.0417 & 0.1490$\pm$0.0791& 0.4176$\pm$0.2612 & 0.2632$\pm$0.2452 & 0.3067$\pm$0.2122\\
\hline
\end{tabular}
}
\end{small}
\end{center}
\end{table*}




% mini-max + rs
% no attack & 0.4422 & 0.2336 & 0.3656\\
% 1 & 0.4692 & 0.2470 & 0.3651\\
% 5 & 0.3877 & 0.2000 & 0.3289\\
% 9 & 0.3359 & 0.1447 & 0.3226\\
% full attack & 0.2978 & 0.1104 & 0.3432\\


==> tables/table_wiki_new.tex <==
\begin{table*}[h]
\caption{Average wQL on electricity dataset under \textbf{deterministic} and \textbf{probabilistic} attack. Target time series $I=\{1\}$ and attacked time stamp $H=\{\tau\}$. Smaller is better.}
\label{table:taxi_new}
\begin{center}
\begin{small}
\scalebox{1}{
\begin{tabular}{c|cccc|cccc}
\hline
 & \multicolumn{4}{c|}{deterministic attack} & \multicolumn{4}{c}{probabilistic attack}\\
\hline
Sparsity & no defense & DA & RS & mini-max & no defense & DA & RS & mini-max\\
\hline
no attack & 0.1645& 0.0868& \textbf{0.0796}& 0.2331 & 0.1645& 0.0868& \textbf{0.0796}& 0.2331\\
1 & 0.2430& 0.0775& \textbf{0.0687}& 0.1683& 0.3255& \textbf{0.1647}& 0.1976& 0.1834\\
3 & 0.2771& 0.2225& 0.2260& \textbf{0.1466}& 0.4080& 0.3104& \textbf{0.2255}& 0.2549\\
5 & 0.4260& 0.3533& 0.3084& \textbf{0.1675}& 0.5336& 0.2759& 0.1714& \textbf{0.1299}\\
7 & 0.5173& 0.4290& 0.4112& \textbf{0.1973} & 0.6547& 0.3940& 0.2656& \textbf{0.2569}\\
9 & 0.6276& 0.4362& 0.4451& \textbf{0.2185}& 0.8463& 0.5140& \textbf{0.2745}& 0.2909\\
\hline
\end{tabular}
}
\end{small}
\end{center}
\end{table*}


==> tables/table_wiki_sparse.tex <==

\begin{table}[h]
\caption{Metrics on Wiki dataset under \textbf{probabilistic} attack. Target time series $I=\{1\}$ and attacked time stamp $H=\{\tau\}$. Smaller is better.}
\begin{center}
\begin{small}
\scalebox{0.5}{
\begin{tabular}{ccccccccccccc}
\hline
 & \multicolumn{3}{c}{no defense} & \multicolumn{3}{c}{data augmentation} & \multicolumn{3}{c}{randomized smoothing} &\multicolumn{3}{c}{mini-max defense}\\
\hline
Sparsity & MAPE & MSE & wQL & MAPE & MSE & wQL & MAPE & MSE & wQL & MAPE & MSE & wQL\\
\hline
no attack & 0.2859$\pm$0.1587 & 0.1145$\pm$0.0945 & 0.1748$\pm$0.1144& 0.0998$\pm$0.0527 & 0.0136$\pm$0.0092 & 0.0837$\pm$0.0432& 0.0949$\pm$0.0569 & 0.0132$\pm$0.0103 & 0.0828$\pm$0.0443& 0.2714$\pm$0.1426 & 0.1001$\pm$0.0706 & 0.2376$\pm$0.1510\\
1 & 0.4806$\pm$0.2747 & 0.3292$\pm$0.2467 & 0.3255$\pm$0.2132& 0.2459$\pm$0.1347 & 0.0841$\pm$0.0773 & 0.1647$\pm$0.1126& 0.2771$\pm$0.1624 & 0.1111$\pm$0.0808 & 0.1976$\pm$0.1274& 0.2065$\pm$0.1370 & 0.0671$\pm$0.0661 & 0.1834$\pm$0.1409\\
3 & 0.6051$\pm$0.1581 & 0.3987$\pm$0.1826 & 0.4080$\pm$0.1724& 0.4253$\pm$0.1913 & 0.2285$\pm$0.1276 & 0.3104$\pm$0.1550& 0.3219$\pm$0.1611 & 0.1374$\pm$0.0938 & 0.2255$\pm$0.1322& 0.3228$\pm$0.1365 & 0.1284$\pm$0.0755 & 0.2549$\pm$0.1530\\
5 & 0.7502$\pm$0.2332 & 0.6335$\pm$0.3677 & 0.5336$\pm$0.2318& 0.4111$\pm$0.1192 & 0.1875$\pm$0.1161 & 0.2759$\pm$0.1368& 0.2558$\pm$0.1559 & 0.0970$\pm$0.1153 & 0.1714$\pm$0.1348& 0.1833$\pm$0.1093 & 0.0491$\pm$0.0570 & 0.1299$\pm$0.0852\\
7 & 0.8620$\pm$0.2836 & 0.8478$\pm$0.3845 & 0.6547$\pm$0.2940& 0.5519$\pm$0.1566 & 0.3365$\pm$0.1865 & 0.3940$\pm$0.1849& 0.3814$\pm$0.1874 & 0.1912$\pm$0.1523 & 0.2656$\pm$0.1708& 0.3441$\pm$0.1938 & 0.1673$\pm$0.1401 & 0.2569$\pm$0.1605\\
9 & 1.0912$\pm$0.2091 & 1.2477$\pm$0.4958 & 0.8463$\pm$0.2715& 0.6810$\pm$0.1719 & 0.5023$\pm$0.2511 & 0.5140$\pm$0.2195& 0.4006$\pm$0.1533 & 0.1911$\pm$0.1223 & 0.2745$\pm$0.1513& 0.3722$\pm$0.2135 & 0.1979$\pm$0.1623 & 0.2909$\pm$0.1918\\
\hline
\end{tabular}
}
\end{small}
\end{center}
\end{table}

